Understanding the Effects of Adversarial Personalized Ranking Optimization Method on Recommendation Quality

Recommender systems (RSs) employ user-item feedback, e.g., ratings, to match customers to personalized lists of products. Approaches to top-k recommendation mainly rely on Learning-To-Rank algorithms and, among them, the most widely adopted is Bayesian Personalized Ranking (BPR), which bases on a pair-wise optimization approach. Recently, BPR has been found vulnerable against adversarial perturbations of its model parameters. Adversarial Personalized Ranking (APR) mitigates this issue by robustifying BPR via an adversarial training procedure. The empirical improvements of APR's accuracy performance on BPR have led to its wide use in several recommender models. However, a key overlooked aspect has been the beyond-accuracy performance of APR, i.e., novelty, coverage, and amplification of popularity bias, considering that recent results suggest that BPR, the building block of APR, is sensitive to the intensification of biases and reduction of recommendation novelty. In this work, we model the learning characteristics of the BPR and APR optimization frameworks to give mathematical evidence that, when the feedback data have a tailed distribution, APR amplifies the popularity bias more than BPR due to an unbalanced number of received positive updates from short-head items. Using matrix factorization (MF), we empirically validate the theoretical results by performing preliminary experiments on two public datasets to compare BPR-MF and APR-MF performance on accuracy and beyond-accuracy metrics. The experimental results consistently show the degradation of novelty and coverage measures and a worrying amplification of bias.

==> Figures/NovRec.tex <==
\begin{figure}[t]
  \centering
    \begin{minipage}[b]{0.195\textwidth}
    \includegraphics[width=\textwidth]{Plots/ML100K/Plot4/Recall_by_alpha-Top50.png}
    \subcaption{$Rec$ - ML100K}
    \label{subfig:ml100k-recall-by-alpha}
  \end{minipage}
  \begin{minipage}[b]{0.195\textwidth}
    \includegraphics[width=\textwidth]{Plots/Amazon/Plot4/Recall_by_alpha-Top50.png}
    \subcaption{$Rec$ - Amazon}
    \label{subfig:amazon-recall-by-alpha}
  \end{minipage}
    \begin{minipage}[b]{0.195\textwidth}
    \includegraphics[width=\textwidth]{Plots/LastFM/Plot4/Recall_by_alpha-Top50.png}
    \subcaption{$Rec$ - Last.fm}
    \label{subfig:lastfm-recall-by-alpha}
  \end{minipage}
  \begin{minipage}[b]{0.195\textwidth}
    \includegraphics[width=\textwidth]{Plots/ML1M/Plot4/Recall_by_alpha-Top50.png}
    \subcaption{$Rec$ - ML1M}
    \label{subfig:ml1m-recall-by-alpha}
  \end{minipage}
\begin{minipage}[b]{0.2\textwidth}
    \includegraphics[width=\textwidth]{Plots/Yelp/Plot4/Recall_by_alpha-Top50.png}
    \subcaption{$Rec$ - Yelp}
    \label{subfig:yelp-recall-by-alpha}
  \end{minipage}
  \begin{minipage}[b]{0.195\textwidth}
    \includegraphics[width=\textwidth]{Plots/ML100K/Plot4/Novelty_by_alpha-Top50.png}
    \subcaption{$Nov$ - ML100K}
    \label{subfig:ml100k-novelty-by-alpha}
  \end{minipage}
    \begin{minipage}[b]{0.195\textwidth}
    \includegraphics[width=\textwidth]{Plots/Amazon/Plot4/Novelty_by_alpha-Top50.png}
    \subcaption{$Nov$ - Amazon}
    \label{subfig:amazon-novelty-by-alpha}
  \end{minipage}
    \begin{minipage}[b]{0.195\textwidth}
    \includegraphics[width=\textwidth]{Plots/LastFM/Plot4/Novelty_by_alpha-Top50.png}
    \subcaption{$Nov$ - Last.fm}
    \label{subfig:lastfm-novelty-by-alpha}
  \end{minipage}
  \begin{minipage}[b]{0.195\textwidth}
    \includegraphics[width=\textwidth]{Plots/ML1M/Plot4/Novelty_by_alpha-Top50.png}
    \subcaption{$Nov$ - ML1M}
    \label{subfig:ml1m-novelty-by-alpha}
  \end{minipage}
    \begin{minipage}[b]{0.2\textwidth}
    \includegraphics[width=\textwidth]{Plots/Yelp/Plot4/Novelty_by_alpha-Top50.png}
    \subcaption{$Nov$ - Yelp}
    \label{subfig:yelp-novelty-by-alpha}
  \end{minipage}
    \begin{minipage}[b]{\textwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/LegendRecNov.png}
  \end{minipage}
  \caption{Plots of the $Rec$ (on the top) and $Rec$ metrics on y-axis by varying $\alpha$ on x-axis. }
    \label{fig:novely-recall}
    \vspace{-1em}
\end{figure}

==> Figures/Pareto-Efficient.tex <==
\begin{figure}[]
    \centering
        \begin{subfigure}[b]{0.8\columnwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Figures/Legend3D.png}
    \end{subfigure}
    % \begin{subfigure}[b]{0.480\columnwidth}   
    %     \centering 
    %     \includegraphics[width=\textwidth]{Figures/Legend2D.png}
    % \end{subfigure}
    \begin{subfigure}[b]{0.480\columnwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Plots/ML100K/Plot5/3D-pareto_Recall-Novelty-APLT-Top50.png}
        \caption[]%
        {{\small ML100K}}    
        \label{subfig:ml100k-pareto-3d}
    \end{subfigure}
    \begin{subfigure}[b]{0.480\columnwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Plots/ML100K/Plot5/pareto_Recall-Novelty-APLT-Top50.png}
        \caption[]%
        {{\small ML100K}}    
        \label{subfig:ml100k-pareto}
    \end{subfigure}
    \begin{subfigure}[b]{0.480\columnwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Plots/LastFM/Plot5/3D-pareto_Recall-Novelty-APLT-Top50.png}
        \caption[]%
        {{\small Last.fm}}    
        \label{subfig:lastfm-pareto-3d}
    \end{subfigure}
    \begin{subfigure}[b]{0.480\columnwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Plots/LastFM/Plot5/pareto_Recall-Novelty-APLT-Top50.png}
        \caption[]%
        {{\small Last.fm}}    
        \label{subfig:lastfm-pareto}
    \end{subfigure}
        \begin{subfigure}[b]{0.480\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Plots/Amazon/Plot5/3D-pareto_Recall-Novelty-APLT-Top50.png}
        \caption[Amazon]%
        {{\small Amazon}}    
        \label{subfig:amazon-pareto-3d}
    \end{subfigure}
    \begin{subfigure}[b]{0.480\columnwidth}  
        \centering 
        \includegraphics[width=\textwidth]{Plots/Amazon/Plot5/pareto_Recall-Novelty-APLT-Top50.png}
        \caption[]%
        {{\small Amazon}}    
        \label{subfig:amazon-pareto}
    \end{subfigure}
    \begin{subfigure}[b]{0.480\columnwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Plots/ML1M/Plot5/3D-pareto_Recall-Novelty-APLT-Top50.png}
        \caption[]%
        {{\small ML1M}}    
        \label{subfig:ml1m-pareto-3d}
    \end{subfigure}
    \begin{subfigure}[b]{0.480\columnwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Plots/ML1M/Plot5/pareto_Recall-Novelty-APLT-Top50.png}
        \caption[]%
        {{\small ML1M}}    
        \label{subfig:ml1m-pareto}
    \end{subfigure}
    \begin{subfigure}[b]{0.480\columnwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Plots/Yelp/Plot5/3D-pareto_Recall-Novelty-APLT-Top50.png}
        \caption[]%
        {{\small Yelp}}    
        \label{subfig:yelp-pareto-3d}
    \end{subfigure}
    \begin{subfigure}[b]{0.480\columnwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Plots/Yelp/Plot5/pareto_Recall-Novelty-APLT-Top50.png}
        \caption[]%
        {{\small Yelp}}    
        \label{subfig:yelp-pareto}
    \end{subfigure}
    \caption{ \small The 3D plot shows the Pareto frontier (in red) of the $Rec$, $Nov$, and $APLT$ objectives. The right plot shows the optimal points. We circled in red the case with $R.V.(\cdot)>0$ for the three metrics.}
    \label{fig:pareto}
\end{figure}

==> Figures/Popularity.tex <==
\begin{figure}[!tbp]
  \centering
      \begin{subfigure}[b]{0.24\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Plots/LastFM/item_popularity_plot.png}
        \caption[Last.fm]%
        {{\small Last.fm}}    
    \end{subfigure}
    \begin{subfigure}[b]{0.24\columnwidth}  
        \centering 
        \includegraphics[width=\textwidth]{Plots/Amazon/item_popularity_plot.png}
        \caption[]%
        {{\small Amazon}}    
    \end{subfigure}
    \begin{subfigure}[b]{0.24\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Plots/ML1M/item_popularity_plot.png}
        \caption[ML1M]%
        {{\small ML1M}}    
    \end{subfigure}
    \begin{subfigure}[b]{0.24\columnwidth}  
        \centering 
        \includegraphics[width=\textwidth]{Plots/Yelp/item_popularity_plot.png}
        \caption[Yelp]%
        {{\small Yelp}}    
    \end{subfigure}
  \caption{\textbf{Imbalanced feedback distributions.} Each
curve is divided in short-head and long-tail items following~\cite{DBLP:conf/recsys/AbdollahpouriBM17}.}
\label{table:item_popularities}
\end{figure}

==> Plots/Dataset-statistics.tex <==
\begin{table}[t]
\caption{The statistics of the datasets.}
\begin{center}
\begin{adjustbox}{width=0.95\columnwidth,center}

\begin{tabular}{|l|r|r|r|r|r|r|}
\hline
\multicolumn{1}{|l|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\textbf{$|U|$}} & \multicolumn{1}{c|}{\textbf{$|I|$}} & \multicolumn{1}{c|}{\small Feedback} & \multicolumn{1}{c|}{\small Density} & \multicolumn{1}{c|}{\textbf{$p(i|I_{SH})$}} & \multicolumn{1}{c|}{\textbf{$p(i|I_{LT})$}} \\ \hline
\textbf{ML100K} & 943 & 1,682 & 99,999 & 0.0630 & 0.6452 & 0.3548 \\ \hline
\textbf{Amazon} & 3,915 & 2,549 & 77,328 & 0.0077 & 0.5747 & 0.4253 \\ \hline
\end{tabular}
\end{adjustbox}
\end{center}
\label{table:datasets}
% \vspace{-0.6cm}
\end{table}


==> Src/Discussion.tex <==
\section{Experimental Evaluation}\label{sec:discussion}
This section presents the results and the discussion of the APR impact on accuracy, beyond-accuracy, and popularity objectives. Here, we aim to answer the following research questions: 
\begin{itemize}
    \item[RQ1.] When APR improves the model accuracy, what are the effects on the beyond accuracy measures? Are the recommendation lists affected by the popularity bias more than the ones produced by BPR? 
    \item[RQ2.] How the $\alpha$ and $\epsilon$ hyper-parameters affect the accuracy and beyond-accuracy of APR performance? 
\end{itemize}

We report all the metric values on top-50 recommendation lists. We indicate $Nov@50$ as $Nov$, $Rec@50$ as $Rec$, $nDCG@50$ as $nDCG$, etc. Additionally, we indicate with $\textbf{R.V.}$ the percentage relative variation between BPR-MF and APR-MF metric values.


\input{Tables/top-50-short}
In this subsection, we aim to verify, what are the effects on the beyond accuracy and popularity bias when APR improves the model accuracy.

\subsubsection{Accuracy and Beyond-Accuracy Performance.}
\Cref{table:accuracy-vs-beyond-vs-bias} shows the accuracy and beyond-accuracy metrics presented in~\Cref{subsec:evaluation-metrics}. For each dataset, we report the model's recommendation performance with the best $Rec$ values in the set of hyper-parameters combinations presented in section~\Cref{subsec:reproducibility}. 

Analyzing~\Cref{table:accuracy-vs-beyond-vs-bias}, we identify that APR tends to reduce the novelty and coverage values compared to the one measured on BPR. For the ML100K dataset, APR-MF improves $Rec$, $Prec$, and $nDCG$ by more than $2\%$, with a slight reduction of $Nov$, i.e., $\textbf{R.V.}(Nov)=-0.27\%$. For Last.fm, we measured an $\textbf{R.V.}(Rec)=+7.14\%$, while a $\textbf{R.V.}(Cov_{\%})=-9.5\%$. Similarly, the ML1M results improve the $Rec$ of 3.62\% while decreasing 6\% the recommendation novelty. The same behavior is even more noticeable for the Yelp results, where the $Cov_{\%}$ got a reduction greater than the $42\%$. Hence, we argue that the APR could negatively influence the beyond-accuracy recommendation performance. 


\subsubsection{Popularity Bias}
\Cref{table:accuracy-vs-beyond-vs-bias} also shows the two groups of metrics to evaluate the popularity bias presented in~\Cref{subsec:evaluation-metrics}. 

\noindent \textbf{1. Long-tail diversity.}
As expected by the analysis in~\Cref{subsec:amplification-bias}, the three long-tail diversity scores get negative \textbf{R.V.} when comparing APR-MF with BPR-MF, its building block. 
Examining the $ARP$ values, we identify that APR-MF results increase the recurrence of most popular items in the recommendation lists. For instance, the $\textbf{R.V.}(ARP)=+23.18\%$ on Amazon, +10.13\% on ML1M, and +32.57\% on Yelp. 
As stated by~\citet{DBLP:conf/flairs/AbdollahpouriBM19}, since the ARP is not a good measure of long-tail diversity when used only on its own, we also report $APLT$ and $ACLT$. For both metrics, the \textbf{R.V.} values are negatives, a behavior consistent with the growth of $ARP$. This empirical evaluation further supports our argument that APR could amplify the popularity bias more than BPR. 

\noindent \textbf{2. Ranking-based statistical item under-recommendation.}
\Cref{table:accuracy-vs-beyond-vs-bias} also reports the $RSP$ and $REO$. While~\citet{DBLP:conf/sigir/ZhuWC20} used these metrics to study the bias on a different group of items based on categorical information, e.g., genres; we studied the items divided into the short-head and long-tail groups (see~\Cref{subsec:amplification-bias} for further details). Consistent with the previous findings, $RSP$ and $REO$ values grew up when employing APR. For instance, $\textbf{R.V.}(RSP)=+3.12\%$ and $\textbf{R.V.}(REO)=+9.69\%$ measured on the ML1M datasets, show that the recommendations are biased towards the short-head items. Variation even bigger on the experiments on the Yelp dataset, e.g., $\textbf{R.V.}(REO)=+15.95\%$. Finally, the comparison between ($P_{SH}, \hat{P}_{SH}$) and ($P_{LT}, \hat{P}_{LT}$) pairs of measures reveal that APR worsened the already discriminatory behavior of BPR on the popular items. For example, the $P_{SH}$ value is 17 times higher than $P_{LT}$ in BPR-MF, while it is 23 times higher in APR-MF for the results on the ML1M dataset. Similarly, the same ratio increases by more than three times in the Yelp dataset.

Before we explore the effects of APR hyper-parameters in~\Cref{subsec:rq2}, we try to connect the results observed in~\Cref{table:accuracy-vs-beyond-vs-bias} together with the dataset characteristics reported in~\Cref{table:datasets}. An interesting finding that we could observe is that Yelp, the dataset with the lowest density ($0.0011$), is the one on which APR had the highest impact of bias amplification and beyond-accuracy performance reduction. Simultaneously, ML1M and ML100K -the two denser datasets- show less evident performance worsening. Indeed, suppose we order the datasets from the smallest to the highest density, we have the following relation $Yelp < Last.fm < Amazon < ML1M < ML100K$. The same order is also present for the $Cov_{\%}$ values and the $APLT$ \textbf{R.V.} - except for a position swap between ML1M and Amazon.

% \subsection{Study of $\alpha$ and $\epsilon$ (RQ2)}~\label{subsec:rq2}
% \input{Figures/NovRec}
% To further study the effect of APR, in this section, we investigate the variation of the adversarial perturbation budget ($\epsilon$) and regularization coefficient ($\alpha$). \Cref{fig:novely-recall} reports the $Rec$ and $Nov$ values evaluated on the ($\alpha,\epsilon$)-model pairs that got the best $Rec$. Additionally, we show the metric value of the most accurate BPR-MF model (straight black line). 

% The ranking accuracy achieved for the APR-MF models with $\epsilon = 1.0$ (straight red line) shows a behavior not comparable to the results obtained with $\epsilon < 1.0$. This behavior confirmed on the $Nov$ plots reveals that the application of adversarial training with big magnitudes of the adversarial perturbation, e.g., $\epsilon \geq 1$ can considerably change the recommendation performance. The negative impact of $\epsilon \geq 1.0$ has also been observed by the original work that proposed the adversarial training strategy~\cite{DBLP:conf/sigir/0001HDC18}. Extending the analysis to  $\epsilon \in \{0.001, 0.01, 0.1\}$, we observe that the $Rec$ values follow the same pattern when we fix the dataset and vary $\alpha$. For instance, APR-MF trained on Amazon leads to $Rec$ values higher than the BPR-MF in the combination $\alpha = 0.01$ and each $\epsilon < 1.0$. The APR accuracy improvements on BPR are verified for each $(\alpha, \epsilon)$-combination on the ML100K dataset (see~\Cref{subfig:ml100k-recall-by-alpha}). Then, we observe the value of APR in the case of the Yelp dataset in~\Cref{subfig:yelp-recall-by-alpha}. In this case, we can see that APR with $\epsilon=1.0$ could produce a model more accurate than the one learned by BPR. Since there is not a clear common pattern across the models trained on the five tested datasets, we conjecture that the performance of APR could depend on the structural and distributional characteristics of the dataset.
% Similar to the findings on $Rec$, the beyond-accuracy values measured with $\alpha = 0.01$ and $\epsilon < 1.0$ have patterns that vary with the dataset. From the novelty plots in~\Cref{fig:novely-recall}, we extract two findings. First, the $(\alpha, \epsilon)$-combinations where the APR accuracy performance is higher than the BPR have not correspondence on the cases where APR can lead to $Nov_{\%}$ improvements on BPR. Second, the APR models' novelty values are mostly lower than those measured on the BPR-MF model. These two observations are in line with the reduction of beyond-accuracy metrics shown in \Cref{table:accuracy-vs-beyond-vs-bias}, and the strict connection between their reduction in the case of amplification of the popularity bias as argued by~\cite{DBLP:journals/ipm/BorattoFM21}.

==> Src/Related.tex <==
\section{Related Work}\label{sec:related}
We now report on the literature related to the application of adversarial learning techniques in recommendation domain and to the key recommendation model features of beyond-accuracy performance and amplification of biases.

\subsection{Models and Evaluation of Adversarial Machine Learning in RSs}
Adversarial Machine Learning (AML) is the field of study of the security for ML models. While the research on the injection of hand-engineered fake profiles has characterized the last twenty years of security investigation of RSs~\cite{DBLP:reference/sp/BurkeOH15}, the recent years view an increase of interest toward AML techniques~\cite{DBLP:conf/nips/LiWSV16, DBLP:conf/sigir/0001HDC18, adversarial2021survey}.
The literature has been focused on three main classes of AML applications: (i) injection of adversarial perturbations on model parameters~\cite{DBLP:conf/sigir/0001HDC18,DBLP:conf/recsys/ChenL19, DBLP:journals/tkde/TangDHYTC20}, (ii) adversarial attacks on the side information, e.g., items' images~\cite{DBLP:conf/dsn/NoiaMM20,cohen2020blackbox,DBLP:journals/corr/abs-2006-01888}, and (iii) AML-optimized data poisoning attacks~\cite{DBLP:conf/nips/LiWSV16,DBLP:conf/recsys/Christakopoulou19} and defenses~\cite{DBLP:conf/wsdm/EntezariADP20, DBLP:conf/sigir/LiuXC0YZ20}. This work falls in the first class. Here, ~\citet{DBLP:conf/sigir/0001HDC18} proposed the pioneering application of AML for the item recommendation task. They reported serious vulnerability of BPR-MF when the model parameters were adversarially perturbed. Additionally, the authors extended BPR with an adversarial training procedure, named adversarial personalized ranking (APR), as an effective defensive countermeasure. This work inspired a series of robustness studies on other core ML models and recommendation tasks. For instance, ~\citet{DBLP:journals/tkde/TangDHYTC20} applied the vulnerability study and proposed the APR defense to a visual-based RS for fashion recommendation. \citet{DBLP:conf/sigir/YuanYB19,DBLP:conf/ijcnn/YuanYB19} investigated the robustification benefits of APR on a class of deep learning recommenders, the collaborative auto-encoder. ~\citet{DBLP:conf/recsys/ChenL19} adopted the same approach to tensor-factorization models. \citet{DBLP:conf/sigir/TranSL19} used APR for automatic playlist continuation. \citet{DBLP:conf/sigir/ManotumruksaY20} implemented APR on a self-attention sequential recommender. In the literature of AML-RS for this class of attacks and defenses, the robustification analysis has been performed for the recommendation accuracy leaving the beyond-accuracy evaluations as a completely uninvestigated research field that is studied by the current work.  

\subsection{The Importance of Beyond-Accuracy and Popularity Bias Impacts on Recommendation}

Due to the large impact of RSs in the society~\cite{DBLP:journals/cacm/Baeza-Yates18, DBLP:conf/recsys/Baeza-Yates20}, a huge research effort has been dedicated to beyond-accuracy objectives~\cite{DBLP:journals/kbs/BobadillaOHG13}. For instance, studying whether the suggested items are novel and cover the complete catalog, and proposing methods to mitigate several types of biases~\cite{DBLP:journals/corr/abs-2010-03240}, e.g., selection bias\cite{DBLP:conf/sigir/Saito20}, exposure bias~\cite{DBLP:conf/sigir/MorikSHJ20}, and popularity bias~\cite{DBLP:conf/recsys/AbdollahpouriBM17, DBLP:conf/recsys/AbdollahpouriMB20}. Indeed, biases could lower the recommendation quality~\cite{DBLP:conf/sigir/CanamaresC18, DBLP:journals/ipm/BorattoFM21}. In particular, the \textit{popularity bias} is responsible of the “rich-get-richer” Matthew effect on RSs. In fact, a popularity-biased RS tends to recommend the most popular items, named \textit{short-head items}, more than the less interacted ones, called \textit{long-tail}~\cite{DBLP:journals/jasis/NikolovLFM19}. 

Controlling and mitigating popularity biases has attracted massive interest in recent years. For instance, \citet{DBLP:conf/recsys/AbdollahpouriBM17} proposed both a regularization framework~\cite{DBLP:conf/recsys/AbdollahpouriBM17} and a re-ranking algorithm~\cite{DBLP:conf/flairs/AbdollahpouriBM19} to increase the coverage of long-tail items in the recommendation lists and reduce the bias amplification.~\citet{DBLP:journals/umuai/JannachLKJ15} proposed to reduce the popularity bias by sampling the training triplets of pair-wise models including a user, an interacted (positive) item, and a not-interacted (negative) item, where the negative one is less popular than the unobserved item. \citet{DBLP:journals/ipm/BorattoFM21} integrated a balanced negative sampling technique with a novel objective function that reduces the biased correlation between the popularity of products and the user-item relevance score.
In addition, BPR, the building block of the APR approach under our investigation, has been proved to amplify the recommendation lists' popularity-biased. For instance, \citet{DBLP:conf/cikm/MansouryAPMB20} empirically identified that BPR is affected by a potent bias propagation phenomenon, \citet{DBLP:conf/sigir/ZhuWC20} measured the vulnerability of BPR to item under-recommendation bias, \citet{DBLP:journals/ipm/BorattoFM21} studied and connected the BPR item popularity bias to the low beyond-accuracy measures, e.g., novelty and coverage. The importance of beyond-accuracy evaluations~\cite{DBLP:journals/tiis/KaminskasB17}, and the related amplification of popularity bias, motivated our extensive investigation on the APR optimization framework. 

==> Tables/Top-50-OLD-Accuracy-and-Beyond.tex <==
% \begin{table}[t]
% \caption{Accuracy and beyond-accuracy metrics evaluated on Top-$50$ recommendation lists.}
% \begin{center}
% \resizebox{\columnwidth}{!}{%

% \begin{tabular}{|l|l|r|r|r|r|r|}
% \hline
% \multicolumn{ 1}{|c|}{\textbf{Dataset}} & \multicolumn{ 1}{c|}{\textbf{Model}} & \multicolumn{ 3}{c|}{\textbf{Accuracy}} & \multicolumn{ 2}{c|}{\textbf{Beyond-accuracy}} \\ \cline{ 3- 7}
% \multicolumn{ 1}{|c|}{} & \multicolumn{ 1}{c|}{} & \multicolumn{1}{c|}{\textit{Rec}} & \multicolumn{1}{c|}{\textit{Prec}} & \multicolumn{1}{c|}{\textit{nDCG}} & \multicolumn{1}{c|}{\textit{Nov}} & \multicolumn{1}{c|}{\textit{$Cov_{\%}$}} \\ \hline

% \multicolumn{ 1}{|c|}{\textbf{ML100K}} & BPR-MF & 0.3871 & 0.0077  & 0.1222 & 2.7653 & 71.22 \\ \cline{ 2- 7}
% \multicolumn{ 1}{|l|}{} & APR-MF& 0.3966  & 0.0079 & 0.1260 & 2.7577 & 71.22 \\ \cline{ 2- 7}
% \multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+2.47\%} & \textbf{+2.47\%} & \textbf{+3.15\%} & \textbf{-0.27\%} & \textbf{+0.00\%} \\ \hline

% \multicolumn{ 1}{|c|}{\textbf{Last.fm}} & BPR-MF  & 0.0148 & 0.0003& 0.0040 & 4.8170 & 20.02 \\ \cline{ 2- 7}
% \multicolumn{ 1}{|l|}{} & APR-MF  & 0.0159& 0.0003 & 0.0042 & 4.7605 & 18.10 \\ \cline{ 2- 7}
% \multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+7.14\%} & \textbf{+7.14\%} & \textbf{3.92\%} & \textbf{-1.17\%} & \textbf{-9.59\%} \\ \hline


% \multicolumn{ 1}{|c|}{\textbf{Amazon}} & BPR-MF & 0.2077  & 0.0042 & 0.0656 & 6.0431 & 99.37 \\ \cline{ 2- 7}
% \multicolumn{ 1}{|l|}{} & APR-MF & 0.2130  & 0.0043 & 0.0687 & 5.6805 & 90.58 \\ \cline{ 2- 7}
% \multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+2.58\%} & \textbf{+2.58\%} & \textbf{+4.63\%} & \textbf{-6.00\%} & \textbf{-8.85\%} \\ \hline


% \multicolumn{ 1}{|c|}{\textbf{ML1M}} & BPR-MF & 0.2747  & 0.0055 & 0.0830 & 2.8576 & 76.19 \\ \cline{ 2- 7}
% \multicolumn{ 1}{|l|}{} & APR-MF & 0.2846 & 0.0057  & 0.0868 & 2.6794 & 70.76 \\ \cline{ 2- 7}
% \multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+3.62\%} & \textbf{+3.62\%} & \textbf{+4.68\%} & \textbf{-6.24\%} & \textbf{-7.13\%} \\ \hline

% \multicolumn{ 1}{|c|}{\textbf{Yelp}} & BPR-MF & 0.0990 & 0.0020 & 0.0290 & 7.7969 & 77.7100 \\ \cline{ 2- 7}
% \multicolumn{ 1}{|l|}{} & AMF & 0.1065 & 0.0021 & 0.0311 & 7.2165 & 44.4300 \\ \cline{ 2- 7}
% \multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+7.55\%} & \textbf{+7.55\%} & \textbf{+7.49\%} & \textbf{-7.44\%} & \textbf{-42.83\%} \\ \hline


% \end{tabular}
% }
% \end{center}
% \label{table:accuracy-vs-beyond}
% \end{table}


% \begin{table*}[!th]
% \caption{Bias measures. The $\uparrow$ means that bigger value is related to an higher popularity bias, $\downarrow$ means less popularity bias.}
% \begin{center}
% \resizebox{0.75\textwidth}{!}{%
% \begin{tabular}{|l|l|r|r|r|r|r|r|r|r|r|}
% \hline
% \multicolumn{ 1}{|c|}{\textbf{Dataset}} & \multicolumn{ 1}{c|}{\textbf{Model}} & \multicolumn{ 3}{c|}{\textbf{Long-tail diversity}} & \multicolumn{ 6}{c|}{\textbf{Ranking-based statistical item under-recommendation}} \\ \cline{ 3- 11}
% \multicolumn{ 1}{|c|}{} & \multicolumn{ 1}{c}{} &      \multicolumn{1}{|c|}{\textit{ARP $\uparrow$}} & 
%      \multicolumn{1}{|c|}{\textit{APLT} $\downarrow$} & 
%      \multicolumn{1}{c|}{\textit{ACLT} $\downarrow$} & 
%      \multicolumn{1}{c|}{\textit{$P_{SH}$ $\uparrow$}}  & 
%      \multicolumn{1}{c|}{\textit{$P_{LT}$ $\downarrow$}} &
%      \multicolumn{1}{c|}{\textit{RSP} $\uparrow$} & 
%      \multicolumn{1}{c|}{\textit{$\hat{P}_{SH}$ $\uparrow$}} &
%      \multicolumn{1}{c|}{\textit{$\hat{P}_{LT}$ $\downarrow$}} &
%      \multicolumn{1}{c|}{\textit{REO} $\uparrow$} \\ \hline

% \multicolumn{ 1}{|c|}{\textbf{ML100K}} & BPR-MF & 176.64 & 0.2890 & 14.4486 & 0.0953 & 0.0102 & 0.8058 & 0.5279 & 0.2167 & 0.4180 \\ \cline{ 2- 11}
% \multicolumn{ 1}{|l|}{} & APR-MF & 177.33* & 0.2841* & 14.2068* & 0.0959* & 0.0101* & 0.8099* & 0.5549* & 0.2048 & 0.4609 \\ \cline{ 2- 11}
% \multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+0.39\%} & \textbf{-1.67\%} & \textbf{-1.67\%} & \textbf{+0.68\%} & \textbf{-1.67\%} & \textbf{+0.51\%} & \textbf{+5.11\%} & \textbf{-5.49\%} & \textbf{+10.26\%} \\ \hline

% \multicolumn{ 1}{|c|}{\textbf{Last.fm}} & BPR-MF & 110.77 & 0.0094 & 0.4704 & 0.0141 & 0.0000 & 0.9948 & 0.0985 & 0.0046 & 0.9116 \\ \cline{ 2- 11}
% \multicolumn{ 1}{|l|}{} & AMF & 114.06* & 0.0069* & 0.3451* & 0.0141* & 0.0000* & 0.9962* & 0.1061 & 0.0046 & 0.9176 \\ \cline{ 2- 11}
% \multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+2.96\%} & \textbf{-26.63\%} & \textbf{-26.63\%} & \textbf{+0.25\%} & \textbf{-26.63\%} & \textbf{+0.14\%} & \textbf{7.69\%} & \textbf{0.00\%} & \textbf{+0.66\%} \\ \hline

% \multicolumn{ 1}{|c|}{\textbf{Amazon}} & BPR-MF & 106.59 & 0.3541 & 17.7055 & 0.0625 & 0.0086 & 0.7572 & 0.3469 & 0.1045 & 0.5371 \\ \cline{ 2- 11}
% \multicolumn{ 1}{|l|}{} & APR-MF & 131.30* & 0.2829* & 14.1471* & 0.0694* & 0.0069* & 0.8191* & 0.3595 & 0.1045 & 0.5496 \\ \cline{ 2- 11}
% \multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+23.18\%} & \textbf{-20.10\%} & \textbf{-20.10\%} & \textbf{+11.02\%} & \textbf{-20.10\%} & \textbf{+8.17\%} & \textbf{+3.63\%} & \textbf{0.00\%} & \textbf{+2.34\%} \\ \hline

% \multicolumn{ 1}{|c|}{\textbf{ML1M}} & BPR-MF & 1,072.48 & 0.1819 & 9.0952 & 0.0512 & 0.0030 & 0.8907 & 0.3850 & 0.1108 & 0.5531 \\ \cline{ 2- 11}
% \multicolumn{ 1}{|l|}{} & APR-MF & 1,181.12* & 0.1405* & 7.0262* & 0.0538* & 0.0023* & 0.9184* & 0.4089* & 0.1001* & 0.6067* \\ \cline{ 2- 11}
% \multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+10.13\%} & \textbf{-22.75\%} & \textbf{-22.75\%} & \textbf{+5.06\%} & \textbf{-22.75\%} & \textbf{+3.12\%} & \textbf{+6.19\%} & \textbf{-9.67\%} & \textbf{+9.69\%} \\ \hline

% \multicolumn{ 1}{|c|}{\textbf{Yelp}} & BPR-MF & 204.64 & 0.1428 & 7.1398 & 0.0083 & 0.0003 & 0.9198 & 0.1552 & 0.0215 & 0.7566 \\ \cline{ 2- 11}
% \multicolumn{ 1}{|l|}{} & AMF & 271.30* & 0.0585* & 2.9264* & 0.0091* & 0.0001* & 0.9693* & 0.1752* & 0.0115* & 0.8773 \\ \cline{ 2- 11}
% \multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+32.57\%} & \textbf{-59.01\%} & \textbf{-59.01\%} & \textbf{+9.83\%} & \textbf{-59.01\%} & \textbf{+5.38\%} & \textbf{+12.93\%} & \textbf{-46.72\%} & \textbf{+15.95\%} \\ \hline

% \multicolumn{11}{l}{\textit{* indicates statistically significant results ($\text{p-value} \leq 0.05$) using the paired-t-test.}}
% \end{tabular}
% }
% \end{center}
% \label{table:popularity-bias}
% \end{table*}


==> Tables/Top-50.tex <==
\begin{table*}[!t]
\caption{Accuracy, beyond-accuracy, and popularity bias metrics evaluated on top-$50$ recommendation lists. The $\uparrow$ means that bigger value is related to an higher popularity bias, $\downarrow$ means less bias.}
\begin{center}
\resizebox{1\textwidth}{!}{%

\begin{tabular}{|l|l|rrr|rr|rrr|rrr|rrr|}
\hline

\multirow{3}{*}{\textbf{Dataset}}  & \multirow{3}{*}{\textbf{Model}}  & \multicolumn{ 3}{c|}{\multirow{2}{*}{\textbf{Accuracy}}} & \multicolumn{ 2}{c|}{\multirow{2}{*}{\textbf{Beyond}}} & \multicolumn{ 9}{c|}{\textbf{Popularity Bias}} \\ \cline{ 8- 16}
\multicolumn{ 1}{|c|}{} & \multicolumn{ 1}{c|}{} & \multicolumn{ 3}{c|}{\textbf{}} & \multicolumn{ 2}{c|}{\textbf{}} & \multicolumn{ 3}{c|}{\textbf{Long-tail diversity}} & \multicolumn{ 6}{c|}{\textbf{Ranking-based statistical item under-recommendation}} \\ \cline{ 3- 16}

% \multicolumn{ 1}{|c|}{\textbf{Dataset}} & \multicolumn{ 1}{c|}{\textbf{Model}} & \multicolumn{ 3}{c|}{\textbf{Accuracy}} & \multicolumn{ 2}{c|}{\textbf{Beyond-accuracy}} & \multicolumn{ 3}{c|}{\textbf{Long-tail diversity}} & \multicolumn{ 6}{c|}{\textbf{Ranking-based statistical item under-recommendation}} \\ \cline{ 3- 16}

\multicolumn{ 1}{|c|}{} & \multicolumn{ 1}{c|}{} & \multicolumn{1}{c}{\textit{Rec}} & \multicolumn{1}{c}{\textit{Prec}} & \multicolumn{1}{c|}{\textit{nDCG}} & \multicolumn{1}{c}{\textit{Nov}} & \multicolumn{1}{c|}{\textit{$Cov_{\%}$}} &      \multicolumn{1}{c}{\textit{ARP $\uparrow$}} & 
     \multicolumn{1}{c}{\textit{APLT} $\downarrow$} & 
     \multicolumn{1}{c|}{\textit{ACLT} $\downarrow$} & 
     \multicolumn{1}{c}{\textit{$P_{SH}$ $\uparrow$}}  & 
     \multicolumn{1}{c}{\textit{$P_{LT}$ $\downarrow$}} &
     \multicolumn{1}{c|}{\textit{RSP} $\uparrow$} & 
     \multicolumn{1}{c}{\textit{$\hat{P}_{SH}$ $\uparrow$}} &
     \multicolumn{1}{c}{\textit{$\hat{P}_{LT}$ $\downarrow$}} &
     \multicolumn{1}{c|}{\textit{REO} $\uparrow$}\\ \hline

\multirow{3}{*}{\textbf{ML100K}} & BPR-MF & 0.3871 & 0.0077  & 0.1222 & 2.7653 & 71.22 & 176.64 & 0.2890 & 14.4486 & 0.0953 & 0.0102 & 0.8058 & 0.5279 & 0.2167 & 0.4180 \\ \cline{ 2- 16}
\multicolumn{ 1}{|l|}{} & APR-MF& 0.3966  & 0.0079 & 0.1260* & 2.7577* & 71.22* & 177.33* & 0.2841* & 14.2068* & 0.0959* & 0.0101* & 0.8099* & 0.5549* & 0.2048 & 0.4609 \\ \cline{ 2- 16}
\multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+2.47\%} & \textbf{+2.47\%} & \textbf{+3.15\%} & \textbf{-0.27\%} & \textbf{0.00\%} & \textbf{+0.39\%} & \textbf{-1.67\%} & \textbf{-1.67\%} & \textbf{+0.68\%} & \textbf{-1.67\%} & \textbf{+0.51\%} & \textbf{+5.11\%} & \textbf{-5.49\%} & \textbf{+10.26\%}\\ \hline

\multirow{3}{*}{\textbf{Last.fm}} & BPR-MF  & 0.0148 & 0.0003& 0.0040 & 4.8170 & 20.02  & 110.77 & 0.0094 & 0.4704 & 0.0141 & 0.0000 & 0.9948 & 0.0985 & 0.0046 & 0.9116\\ \cline{ 2- 16}
\multicolumn{ 1}{|l|}{} & APR-MF  & 0.0159& 0.0003 & 0.0042 & 4.7605 & 18.10 & 114.06* & 0.0069* & 0.3451* & 0.0141* & 0.0000* & 0.9962* & 0.1061 & 0.0046 & 0.9176\\ \cline{ 2- 16}
\multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+7.14\%} & \textbf{+7.14\%} & \textbf{3.92\%} & \textbf{-1.17\%} & \textbf{-9.59\%} & \textbf{+2.96\%} & \textbf{-26.63\%} & \textbf{-26.63\%} & \textbf{+0.25\%} & \textbf{-26.63\%} & \textbf{+0.14\%} & \textbf{7.69\%} & \textbf{0.00\%} & \textbf{+0.66\%}\\ \hline


\multirow{3}{*}{\textbf{Amazon}} & BPR-MF & 0.2077  & 0.0042 & 0.0656 & 6.0431 & 99.37 & 106.59 & 0.3541 & 17.7055 & 0.0625 & 0.0086 & 0.7572 & 0.3469 & 0.1045 & 0.5371  \\ \cline{ 2- 16}
\multicolumn{ 1}{|l|}{} & APR-MF & 0.2130  & 0.0043 & 0.0687* & 5.6805* & 90.58* & 131.30* & 0.2829* & 14.1471* & 0.0694* & 0.0069* & 0.8191* & 0.3595 & 0.1045 & 0.5496 \\ \cline{ 2- 16}
\multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+2.58\%} & \textbf{+2.58\%} & \textbf{+4.63\%} & \textbf{-6.00\%} & \textbf{-8.85\%} & \textbf{+23.18\%} & \textbf{-20.10\%} & \textbf{-20.10\%} & \textbf{+11.02\%} & \textbf{-20.10\%} & \textbf{+8.17\%} & \textbf{+3.63\%} & \textbf{0.00\%} & \textbf{+2.34\%}\\ \hline


\multirow{3}{*}{\textbf{ML1M}} & BPR-MF & 0.2747  & 0.0055 & 0.0830 & 2.8576 & 76.19 & 1,072.48 & 0.1819 & 9.0952 & 0.0512 & 0.0030 & 0.8907 & 0.3850 & 0.1108 & 0.5531\\ \cline{ 2- 16}
\multicolumn{ 1}{|l|}{} & APR-MF & 0.2846* & 0.0057*  & 0.0868* & 2.6794* & 70.76* & 1,181.12* & 0.1405* & 7.0262* & 0.0538* & 0.0023* & 0.9184* & 0.4089* & 0.1001* & 0.6067*\\ \cline{ 2- 16}
\multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+3.62\%} & \textbf{+3.62\%} & \textbf{+4.68\%} & \textbf{-6.24\%} & \textbf{-7.13\%} & \textbf{+10.13\%} & \textbf{-22.75\%} & \textbf{-22.75\%} & \textbf{+5.06\%} & \textbf{-22.75\%} & \textbf{+3.12\%} & \textbf{+6.19\%} & \textbf{-9.67\%} & \textbf{+9.69\%}\\ \hline

\multirow{3}{*}{\textbf{Yelp}} & BPR-MF & 0.0990 & 0.0020 & 0.0290 & 7.7969 & 77.71  & 204.64 & 0.1428 & 7.1398 & 0.0083 & 0.0003 & 0.9198 & 0.1552 & 0.0215 & 0.7566  \\ \cline{ 2- 16}
\multicolumn{ 1}{|l|}{} & APR-MF & 0.1065* & 0.0021* & 0.0311* & 7.2165* & 44.43* & 271.30* & 0.0585* & 2.9264* & 0.0091* & 0.0001* & 0.9693* & 0.1752* & 0.0115* & 0.8773 \\ \cline{ 2- 16}
\multicolumn{ 1}{|l|}{} & \multicolumn{1}{r|}{\textbf{R.V.}} & \textbf{+7.55\%} & \textbf{+7.55\%} & \textbf{+7.49\%} & \textbf{-7.44\%} & \textbf{-42.83\%}  & \textbf{+32.57\%} & \textbf{-59.01\%} & \textbf{-59.01\%} & \textbf{+9.83\%} & \textbf{-59.01\%} & \textbf{+5.38\%} & \textbf{+12.93\%} & \textbf{-46.72\%} & \textbf{+15.95\%}\\ \hline

\multicolumn{16}{l}{\textit{* indicates statistically significant results ($\text{p-value} \leq 0.05$) using the paired-t-test.}}

\end{tabular}
}
\end{center}
\label{table:accuracy-vs-beyond-vs-bias}
\vspace{-0.6cm}
\end{table*}


==> Tables/papers.tex <==
% \begin{table}[t]
% \caption{List of retrieved articles that implements APR as the optimization strategy.}
% \begin{adjustbox}{width=\linewidth}
% \begin{tabular}{|l|l|l|r|}
% \hline
% \textbf{Title} & \textbf{Reference}  & \textbf{Conference}  & \textbf{Year} \\ \hline
% Adversarial Personalized Ranking for Recommendation & \citet{DBLP:conf/sigir/0001HDC18} & SIGIR & 2018 \\ \hline
% Adversarial Collaborative Auto-encoder for Top-N Recommendation& \citet{DBLP:conf/ijcnn/YuanYB19} & IJCNN & 2019 \\ \hline
% Adversarial Collaborative Neural Network for Robust Recommendation& \citet{DBLP:conf/sigir/YuanYB19} & SIGIR & 2019 \\ \hline
% Adversarial Mahalanobis Distance-based Attentive Song Recommender for Automatic Playlist Continuation& \citet{DBLP:conf/sigir/TranSL19} & SIGIR & 2019 \\ \hline
% Adversarial Tensor Factorization for Context-aware Recommendation& \citet{DBLP:conf/recsys/ChenL19} & RecSys & 2019 \\ \hline
% Adversarial Sampling and Training for Semi-Supervised Information Retrieval& \citet{DBLP:conf/www/ParkC19} & WWW & 2019 \\ \hline
% Adversarial Training Methods for Network Embedding& \citet{DBLP:conf/www/DaiSZLW19} & WWW & 2019 \\ \hline
% Graph Adversarial Training: Dynamically Regularizing Based on Graph Structure& \citet{8924766} & TKDE & 2019 \\ \hline
% Multi-feedback Pairwise Ranking via Adversarial Training for Recommender& \citet{https://doi.org/10.1049/cje.2020.05.004} & IET & 2019 \\ \hline
% Adversarial Training for Session-based Item Recommendations& \citet{9338819} & IEEE ITAIC & 2019 \\ \hline
% Sequential-based Adversarial Optimisation for Personalised Top-N Item Recommendation& \citet{DBLP:conf/sigir/ManotumruksaY20} & SIGIR & 2020 \\ \hline
% Adversarial Learning to Compare: Self-Attentive Prospective Customer Recommendation in Location based Social Networks& \citet{DBLP:conf/wsdm/LiW020} & WSDM  & 2020 \\ \hline
% Exploring Missing Interactions: A Convolutional Generative Adversarial Network for Collaborative Filtering& \citet{DBLP:conf/cikm/YuanYB20} & WSDM  & 2020 \\ \hline
% Adversarial Training-Based Mean Bayesian Personalized Ranking for Recommender System& \citet{DBLP:journals/access/WangH20a} & IEEE Access & 2020 \\ \hline
% Adversarial Training Towards Robust Multimedia& \citet{DBLP:journals/tkde/TangDHYTC20} & TKDE & 2020 \\ \hline
% % Robust Graph Convolutional Networks with Directional Graph Adversarial Training& \citet{Hu2021} & Applied Intelligence & 2021 \\ \hline
% \end{tabular}
% \end{adjustbox}
% \label{table:papers}
% \end{table}


% \begin{table}[t]
% \caption{List of retrieved articles that implements APR as the optimization strategy.}
% \begin{tabular}{|l|l|r|}
% \hline
% \textbf{Article}  & \textbf{Conference}  & \textbf{Year} \\ \hline
% \citet{DBLP:conf/sigir/0001HDC18} & SIGIR & 2018 \\ \hline
% \citet{DBLP:conf/ijcnn/YuanYB19} & IJCNN & 2019 \\ \hline
% \citet{DBLP:conf/sigir/YuanYB19} & SIGIR & 2019 \\ \hline
% \citet{DBLP:conf/sigir/TranSL19} & SIGIR & 2019 \\ \hline
% \citet{DBLP:conf/recsys/ChenL19} & RecSys & 2019 \\ \hline
% \citet{DBLP:conf/www/ParkC19} & WWW & 2019 \\ \hline
% \citet{DBLP:conf/www/DaiSZLW19} & WWW & 2019 \\ \hline
% \citet{8924766} & TKDE & 2019 \\ \hline
% \citet{https://doi.org/10.1049/cje.2020.05.004} & IET & 2019 \\ \hline
% \citet{9338819} & IEEE ITAIC & 2019 \\ \hline
% \citet{DBLP:conf/sigir/ManotumruksaY20} & SIGIR & 2020 \\ \hline
% \citet{DBLP:conf/wsdm/LiW020} & WSDM  & 2020 \\ \hline
% \citet{DBLP:conf/cikm/YuanYB20} & WSDM  & 2020 \\ \hline
% \citet{DBLP:journals/access/WangH20a} & IEEE Access & 2020 \\ \hline
% \citet{DBLP:journals/tkde/TangDHYTC20} & IEEE TKDE & 2020 \\ \hline
% \citet{Hu2021} & Applied Intelligence & 2021 \\ \hline
% \end{tabular}
% \label{table:papers}
% \end{table}

\begin{table}[t]
\caption{List of articles proposing novel recommendation algorithms employing APR as the optimization strategy.}
\begin{tabular}{|l|l|r|}
\hline
\textbf{Article}  & \textbf{Conference}  & \textbf{Year} \\ \hline
\citet{DBLP:conf/sigir/0001HDC18} & SIGIR & 2018 \\ \hline
\citet{DBLP:conf/ijcnn/YuanYB19} & IJCNN & 2019 \\ \hline
\citet{DBLP:conf/sigir/YuanYB19} & SIGIR & 2019 \\ \hline
\citet{DBLP:conf/sigir/TranSL19} & SIGIR & 2019 \\ \hline
\citet{DBLP:conf/recsys/ChenL19} & RecSys & 2019 \\ \hline
\citet{DBLP:conf/www/ParkC19} & WWW & 2019 \\ \hline
\citet{DBLP:conf/www/DaiSZLW19} & WWW & 2019 \\ \hline
\citet{8924766} & TKDE & 2019 \\ \hline
\citet{https://doi.org/10.1049/cje.2020.05.004} & IET & 2019 \\ \hline
\citet{9338819} & IEEE ITAIC & 2019 \\ \hline
Manotumruksa et al.~\cite{DBLP:conf/sigir/ManotumruksaY20} & SIGIR & 2020 \\ \hline
\citet{DBLP:conf/wsdm/LiW020} & WSDM  & 2020 \\ \hline
\citet{DBLP:conf/cikm/YuanYB20} & WSDM  & 2020 \\ \hline
\citet{DBLP:journals/access/WangH20a} & IEEE Access & 2020 \\ \hline
\citet{DBLP:journals/tkde/TangDHYTC20} & IEEE TKDE & 2020 \\ \hline
\citet{Hu2021} & Applied Intelligence & 2021 \\ 
\hline
\end{tabular}
\label{table:papers}
\end{table}
